Operationalising Rawlsian Ethics for Fairness in Norm-Learning Agents

Social norms are standards of behaviour common in a society. However, when agents make decisions without considering how others are impacted, norms can emerge that lead to the subjugation of certain agents. We present RAWL-E, a method to create ethical norm-learning agents. RAWL-E agents operationalise maximin, a fairness principle from Rawlsian ethics, in their decision-making processes to promote ethical norms by balancing societal well-being with individual goals. We evaluate RAWL-E agents in simulated harvesting scenarios. We find that norms emerging in RAWL-E agent societies enhance social welfare, fairness, and robustness, and yield higher minimum experience compared to those that emerge in agent societies that do not implement Rawlsian ethics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tikz/norms-baseline.tex <==
\usepackage{forest}

\forestset{
  declare forest style named=base_node,
  base_node = [draw, circle, minimum size=3mm],
  % Define styles for different conditions
  health_high = [base_node, fill=green!20],
  health_medium = [base_node, fill=yellow!20],
  health_low = [base_node, fill=red!20],
  berries_high = [base_node, fill=blue!20],
  berries_medium = [base_node, fill=cyan!20],
  berries_no = [base_node],
  days_high = [base_node, fill=orange!20],
  days_medium = [base_node],
  days_low = [base_node, fill=gray!20],
  text action = [right],  % Place action text on the right
}

\newcommand{\parseTreeNode}[1]{%
  \noexpand\forest ([%
    \ifcat\relax#1\relax health_high \else \fi
    \ifcat\relax#1\relax health_medium \else \fi
    \ifcat\relax#1\relax health_low \else \fi
    \ifcat\relax#1\relax berries_high \else \fi
    \ifcat\relax#1\relax berries_medium \else \fi
    \ifcat\relax#1\relax berries_no \else \fi
    \ifcat\relax#1\relax days_high \else \fi
    \ifcat\relax#1\relax days_medium \else \fi
    \ifcat\relax#1\relax days_low \else \fi
    #1, text action=THEN: [#1]
  ])%
}

\begin{document}
\begin{forest}

  % Call the macro for each line in your text file
  \parseTreeNode{medium health}
    \parseTreeNode{no berries}
      \parseTreeNode{low days [move]}
      \parseTreeNode{medium days [move]}
    \parseTreeNode{medium berries}
      \parseTreeNode{medium days [move]}
      \parseTreeNode{low days [eat]}
  \parseTreeNode{high health}
    \parseTreeNode{medium berries}
      \parseTreeNode{high days [eat]}
      \parseTreeNode{medium days [eat]}
    \parseTreeNode{high berries}
      \parseTreeNode{high days [move]}
  % ... (Add similar lines for other health conditions)
\end{forest}
\end{document}
